VI-OOD: A Unified Representation Learning Framework for Textual Out-of-distribution Detection

Out-of-distribution (OOD) detection plays a crucial role in ensuring the safety and reliability of deep neural networks in various applications. While there has been a growing focus on OOD detection in visual data, the field of textual OOD detection has received less attention. Only a few attempts have been made to directly apply general OOD detection methods to natural language processing (NLP) tasks, without adequately considering the characteristics of textual data. In this paper, we delve into textual OOD detection with Transformers. We first identify a key problem prevalent in existing OOD detection methods: the biased representation learned through the maximization of the conditional likelihood $p(y\mid x)$ can potentially result in subpar performance. We then propose a novel variational inference framework for OOD detection (VI-OOD), which maximizes the likelihood of the joint distribution $p(x, y)$ instead of $p(y\mid x)$. VI-OOD is tailored for textual OOD detection by efficiently exploiting the representations of pre-trained Transformers. Through comprehensive experiments on various text classification tasks, VI-OOD demonstrates its effectiveness and wide applicability. Our code has been released at \url{https://github.com/liam0949/LLM-OOD}.

==> 4.exp.tex <==
In this section, we present a comprehensive evaluation of textual out-of-distribution (OOD) detection with pervasive OOD detection methods.
Besides, we demonstrate the effectiveness of our proposed OOD detection method on challenging natural language understanding benchmarks. To achieve a comprehensive evaluation, we employ both encoder-based and decoder-based pre-trained language models as backbone models of our method.
We start this section by describing our evaluation methodology and then present our experimental results.


\subsection{Evaluation Methodology}\label{baselines}

\subsubsection{Datasets}\label{sec:dataset}
OOD detection in the natural language processing (NLP) domain is generally under-explored and only discussed in limited scenarios such as out-of-scope intent detection in dialogue machines~\cite{DCL, ADB, DBLP:conf/acl/YanFLLZWL20}. As such, evaluating OOD performance in the NLP domain does not have a consensus. 
To scale the evaluation process as general as possible, we follow the evaluation in \cite{hendrycks2020pretrained} and \cite{zhou2021contrastive} to present our main analysis. 
% Moreover, we also provide experimental results for OOD intent detection.
 \citet{hendrycks2020pretrained} firstly proposes to use the sentiment analysis benchmark SST-2 as the in-distribution dataset and select five other datasets as out-distribution evaluation sets, which includes 20 Newsgroups, WMT16 and Multi30K, RTE, and SNLI. \citet{zhou2021contrastive} further extend this benchmark by adding more natural language understanding tasks including topic classification, and question classification. 

\paragraph{In-distribution Tasks}
We use four benchmark datasets as in-distribution (ID) tasks: 20 Newsgroups (20NG)~\cite{DBLP:conf/icml/Lang95}, IMDB~\cite{maas2011learning}, SST-2~\cite{socher2013recursive} and TREC-10~\cite{li2002learning}. When setting each of them as \emph{in-distribution}, other ones are recognized as \emph{out-distribution}.
% \begin{itemize}
% \item 20 Newsgroups (20NG)~\cite{DBLP:conf/icml/Lang95} is a commonly used benchmark for the topic (or newsgroup) classification. In this dataset, these are $20$ labeled topic classes and $15,056$, $1,876$, and $1,896$ examples for the train, validation, and test respectively.

% \item IMDB~\cite{maas2011learning} contains $ 25,000$ movie reviews from IMDB which are collected for the task of binary sentiment analysis.  $10\%$ examples are randomly selected as the validation set. 

% \item SST-2~\cite{socher2013recursive} is also a binary sentiment analysis task derived from the Stanford Sentiment Treebank. It consists of $67,349$, $872$ and $1,821$ examples for training, validation and test sets respectively. Note that since both IMDB and SST-2 are sentiment analysis datasets, they are not considered as OOD counterparts in our experiments.

% \item TREC-10~\cite{li2002learning} is a dataset for question classification, which is a preliminary task for question answering. We also use the $6$-class version as \cite{zhou2021contrastive} did. The splitting is $4,907$ for training, $545$ for validation, and $545$ for test.
% \end{itemize}

Besides the above ID four tasks, we also use another four unrelated datasets as OOD test sets (not for training) for all of the four ID tasks. We refer them as the out-distribution datasets: the English source side of English-German WMT16~\cite{bojar-etal-2016-findings} and English-German Multi30K~\cite{elliott2016multi30k}, and concatenations of the premise and hypothesis of RTE~\cite{dagan2006pascal} and MNLI~\cite{williams2018broad}. WMT16 and Multi30K are for machine translation while RTE and MNLI are for natural language inference.
We use the respective test sets of each out-distribution dataset to measure OOD performance.
% \begin{figure*}[t]
% \begin{subfigure}{0.495\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/layers/20ng.png}
%   \caption{ }
%   \label{fig:layer_20ng}
% \end{subfigure}%
% \begin{subfigure}{0.495\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/layers/mnli.png}
%   \caption{}
%   \label{fig:layer_mnli}
% \end{subfigure}

% \begin{subfigure}{.495\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/layers/multi30k.png}
%   \caption{}
%   \label{fig:layer_multi30k}
% \end{subfigure}%
% \begin{subfigure}{.495\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/layers/rte.png}
%   \caption{}
%   \label{fig:layer_rte}
% \end{subfigure}

% \begin{subfigure}{.495\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/layers/trec.png}
%   \caption{}
%   \label{fig:layer_trec}
% \end{subfigure}%
% \begin{subfigure}{.495\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/layers/wmt16.png}
%   \caption{}
%   \label{fig:layer_wmt16}
% \end{subfigure}
% \caption{AUROC results across $24$ layers of RoBERTa\textsubscript{LARGE}. The model is fine-tuned on SST-2 and test OOD performance on 20NG, MNLI and Multi30K, RTE and TREC, WMT16.
% % (a), (b), and (c) display overall accuracy, f1-score on the unknown class and overall macro f1-score with varying number of self-supervised outliers respectively. 
% %Sub-figures \ref{fig:open_domain_acc}, \ref{fig:open_domain_f1_unknown} and \ref{fig:open_domain_f1} 
% % (d), (e), and (f) display the corresponding results with varying number of open-domain outliers.
% }
% % ,,
% \label{fig:layers}
% \end{figure*}

% \begin{figure*}[t]
% \begin{subfigure}{1\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth, height=6cm]{figures/layers/20ng.png}
%   \caption{ }
%   \label{fig:layer_20ng}
% \end{subfigure}

% \begin{subfigure}{1\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth,height=6cm]{figures/layers/mnli.png}
%   \caption{}
%   \label{fig:layer_mnli}
% \end{subfigure}

% \begin{subfigure}{1\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth,height=5cm]{figures/layers/multi30k.png}
%   \caption{}
%   \label{fig:layer_multi30k}
% \end{subfigure}

% \begin{subfigure}{1\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth,height=5cm]{figures/layers/rte.png}
%   \caption{}
%   \label{fig:layer_rte}
% \end{subfigure}

% \begin{subfigure}{.495\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/layers/trec.png}
%   \caption{}
%   \label{fig:layer_trec}
% \end{subfigure}%
% \begin{subfigure}{.495\textwidth}
%   \centering
%   \includegraphics[width=1.\linewidth]{figures/layers/wmt16.png}
%   \caption{}
%   \label{fig:layer_wmt16}
% \end{subfigure}
% \caption{A study on the OOD performance of the intermediate hidden sates. AUROC results across $24$ layers of RoBERTa\textsubscript{LARGE} are reported. The model is fine-tuned on SST-2 and evaluates OOD performance on 20NG and MNLI.
% % (a), (b), and (c) display overall accuracy, f1-score on the unknown class and overall macro f1-score with varying number of self-supervised outliers respectively. 
% %Sub-figures \ref{fig:open_domain_acc}, \ref{fig:open_domain_f1_unknown} and \ref{fig:open_domain_f1} 
% % (d), (e), and (f) display the corresponding results with varying number of open-domain outliers.
% }
% % ,,
% \label{fig:layers}
% \end{figure*}
 
\subsubsection{Baselines}\label{sec:baselines}
To demonstrate the effectiveness of our proposed framework, we compare our method comprehensively with four commonly used OOD detection algorithms:
% namely Maximum Softmax Probability (MSP)~\citep{DBLP:conf/iclr/HendrycksG17}, Mahalanobis Distance (Maha)~\citep{DBLP:conf/nips/LeeLLS18}, Energy score (Energy)~\citep{DBLP:conf/nips/LiuWOL20} and Cosine distance (Cosine)~\citep{zhou2021contrastive}. Additionally, we present the results achieved by executing the code released by \citet{zhou2021contrastive} with the identical random seeds employed in our method. For more detailed information regarding the baselines and datasets, please refer to Appendix~\ref{sec:baselines}.

% MSP~\citep{DBLP:conf/iclr/HendrycksG17}, DOC~\citep{DBLP:conf/emnlp/ShuXL17}, LMCL~\citep{LMCL}, SEG~\citep{SEG}, ADB~\citep{Zhang_Xu_Lin_2021}, and DCL~\citep{DCL}.
\begin{itemize}
\item \textbf{Maximum Softmax Probability (MSP)}~\citep{DBLP:conf/iclr/HendrycksG17}: The MSP confidence score leverages the maximum softmax probability outputted by the softmax function for out-of-domain detection. As correct samples tend to have higher probability scores, samples below a threshold are more likely to be outliers. Specifically, the confidence score is $\mathcal{C}(x) = \max_{y}p(y|x)$.

\item \textbf{Mahalanobis Distance (Maha)}~\citep{DBLP:conf/nips/LeeLLS18}: The Mahalanobis Distance (MD) method fits $K$-class conditional Gaussian
distributions $\{\mathcal{N}(\mu_{i},\Sigma)\}_{i=1}^{K}$ for the $K$ in-distribution classes upon the output of the penultimate layer in the model. The Mahalanobis Distance and the MD confidence score are computed by:
\begin{flalign}
\begin{aligned}\label{eq:md}
\text{MD}_{k}(z) &= (z-\mu_{k})^{T}\Sigma^{-1}(z-\mu_{k}),\\
 \mathcal{C}(x) &=-\min_{k}\{\text{MD}_{k}(z)\}.
\end{aligned}
\end{flalign}

\item \textbf{Energy score (Energy)} \citep{DBLP:conf/nips/LiuWOL20}: The energy score confidence score is inspired by the energy-based models~\cite{lecun2006tutorial}. It defines an energy of an input $(x, y)$ as $E(x, y) = w_{y}^{T} \cdot z$, where $w_{y}$ is the weight of the softmax layer for the $y^{th}$ in-distribution class. The energy score confidence score is defined as:
\begin{flalign}
\begin{aligned}\label{eq:md}
\mathcal{C}(x) = \log \sum_{i}^{K} e^{w_{i}^{T} \cdot z}.
\end{aligned}
\end{flalign}

\item \textbf{Cosine distance (Cosine)}~\citep{zhou2021contrastive}: The cosine distance OOD confidence sore defines as the maximum cosine similarity of a test input representation with representations in the validation set, i.e., $\mathcal{C}(x) = -\max_{i=1}^{V}\text{cos}(z, z_{i}^{val})$.
\end{itemize}

% \begin{table*}[ht!]
% \centering
% \scalebox{0.6}{
% \begin{tabular}{c|c|ccc|ccc|ccc|ccc}
% \specialrule{0.1em}{0.2em}{0.2em}
%  &  &  \multicolumn{3}{c}{\bf SST-2} & \multicolumn{3}{c}{\bf IMDB}&  \multicolumn{3}{c}{\bf TREC-10} & \multicolumn{3}{c}{\bf 20NG}\\
% Methods& Avg. &  AUROC  \uparrow  & FAR@95  \downarrow& AUPR \uparrow &  AUROC  \uparrow  & FAR@95 \downarrow & AUPR \uparrow& AUROC \uparrow & FAR@95 \downarrow& AUPR \uparrow & AUROC  \uparrow  & FAR@95  \downarrow & AUPR \uparrow\\
% \specialrule{0.05em}{0.1em}{0.2em}
% \multirow{4}{*}{}
%                     \bf MSP& 94.0 \slash 36.76 \slash 90.46 & 89.85& 66.2 & 86.4 & 94.3& 41.9 & 98.8 & 97.94 & 8.43 & 89.26 & 93.89 & 30.49& 87.39 \\
%                     \bf Maha& 98.78 \slash6.21\slash97.07 & 97.98& 11.5 & 97.3 & 99.67& 0.7 & 99.95& 98.99 & 4.87 & 95.11& 98.39 & 7.77&95.91 \\
%                     \bf Cosine& 97.94\slash	9.745\slash94.45 & 95.65& 22.65& 94.68& 99.5& 1.53 &99.88& 98.89 & 3.96 & 94.54& 97.73 & 10.84 & 88.71 \\
%                     \bf Energy& 94.01\slash37.93\slash89.01& 89.8& 67 &86.53& 93.3& 56.7&98.63& 97.19 & 10.07 &82.16 & 95.76& 17.93&88.71 \\                  
 
% \specialrule{0.1em}{0.2em}{0.2em}
% \multirow{4}{*}{}
%                     \bf MSP\textsubscript{VI}& 95.25\slash 27.0\slash 89.83& 92.85& 51.58&89.72& 95.95& 28.03&99.12& 98.91 & 2.77 &90.39& 93.29 & 25.61& 80.09 \\
%                     \bf Maha\textsubscript{VI}& 99.62\slash 1.31\slash 98.77 & 99.33& 3.62&98.52& 99.9&0.21& 99.97& 99.46 & 0.79 & 97.67& 99.8 & 0.61&98.93 \\
%                     \bf Cosine\textsubscript{VI}& 99.3\slash3.04\slash97.81 & 98.87& 6.62&98.06& 99.57&1.43 &99.88& 99.36 & 1.19&96.09 & 99.39 & 2.92&97.19 \\
%                     \bf Energy\textsubscript{VI}&95.6\slash24.78\slash89.72 & 92.79& 51.25&89.26& 96.05& 27.97&99.12& 99.21& 2.84 &90.84& 94.34 & 17.04&79.67 \\
% \specialrule{0.1em}{0.2em}{0.2em}

% \end{tabular}
% }
% \caption{\label{tab:main}
% Main results.
% }
% \end{table*}



\subsubsection{Metrics}
We employ three commonly used metrics for OOD detection and introduce them as follows:
\begin{itemize}
\item \textbf{AUROC}: Area Under the Receiver Operating Characteristic
curve(AUROC) reveals the relationship between True Positive Rate (TPR) (i.e., Recall) and False Positive Rate (FPR). It represents the probability of assigning a higher score to a positive example than a negative example. The pioneering work \cite{DBLP:conf/iclr/HendrycksG17} firstly proposed to use this metric for OOD detection. A higher AUROC score indicates a better classifier, and An AUROC score of $50\%$ means random guessing. 

\item \textbf{FAR@95}: False Alarm Rate at $95\%$ Recall(FAR@95) is the probability that a negative example is misclassified as positive when Recall or TPR is $95\%$. In this paper, we take the OOD class as negative.
\item \textbf{AUPR}: Area Under the Precision-Recall curve (AUPR) is another commonly used metric based on the Precision-Recall Curve. It is a better indicator in the case of imbalanced in- and out-rate \cite{manning1999foundations}. A perfect classifier has an AUPR of $100\%$.
\end{itemize}



\subsubsection{Experimental Setup}
For the encoder-based pre-trained language model, we employ the RoBERTa\textsubscript{LARGE}~\cite{liu2019roberta} model from HuggingFace~\cite{wolf2019huggingface} as the backbone of our framework. We use the optimizer AdamW~\cite{DBLP:conf/iclr/LoshchilovH19} with a linear-scheduled learning rate $10^{-5}$ to fine-tune the model for $20$ epochs. For the variational terms in Eq.~\ref{eq:final_loss}, we apply a linear annealing strategy which is a common practice in variational methods~\cite{DBLP:conf/naacl/FuLLGCC19}. All reported results are obtained in $5$ runs with different random seeds.
% For the decoder-based large language model, we verify the effectiveness of our method on LLaMA-2-7B. To boost the fine-tuning process, We perform parameter-effective fine-tuning via the LoRA module provided by the Hugginface PEFT package, and our hyperparameters for LoRA are: $\alpha=16, r=16$ and $lora_dropout=0.05$. We tune the model for $20$ epochs and set the learning rate as $1e-4$. For other training details, please refer to our aforementioned released code repository. 

For the decoder-based large language model, we validate the effectiveness of our method on LLaMA-2-7B. To reduce training costs, we perform parameter-effective fine-tuning through the LoRA module provided by the HuggingFace PEFT package. Our hyperparameters for LoRA are set as follows: $\alpha=16$, $r=16$, and $lora_dropout=0.05$. We fine-tune the model for $20$ epochs with a learning rate of $1e-4$. For additional training details, please refer to the code repository we have released.



% \paragraph{Different baselines have peaked OOD performance in }

\begin{table*}[ht!]
\centering
\scalebox{0.68}{
\begin{tabular}{ccccccc}
\specialrule{0.15em}{0.1em}{0.1em}

 &  \multicolumn{3}{c}{\bf SST-2} & \multicolumn{3}{c}{\bf IMDB}\\
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
Methods & \makecell[c]{AUROC  \uparrow}  & \makecell[c]{FAR@95  \downarrow}& \makecell[c]{AUPR \uparrow} &  \makecell[c]{AUROC  \uparrow}  & \makecell[c]{FAR@95 \downarrow} & \makecell[c]{AUPR \uparrow}\\
\specialrule{0.1em}{0.1em}{0.1em}

    MSP&  89.85& 66.20 & 86.40 & 94.30& 41.90 & 98.80 \\
    MSP\textsubscript{Contrast} & 85.04 & 63.42 & 69.34 & 94.51 & 44.69 & 98.89 \\
\bf MSP\textsubscript{VI}& \bf 92.85 & \bf51.58 &\bf 89.72 & \bf 95.95 & \bf 28.03 &\bf 99.12 \\
\specialrule{0.05em}{0.2em}{0.2em}
    Maha& 97.98& 11.50 & 97.30 & 99.67& 0.70 & 99.95 \\
    Maha\textsubscript{Contrast} & \bf99.42 & \bf2.98 & \bf98.73 & 99.89 & \bf0.05 & \bf99.97 \\
\bf Maha\textsubscript{VI}& 99.33 & 3.62\hspace{0.5em} &98.52 & \bf99.90 & 0.21\hspace{0.5em} & \bf99.97  \\
\specialrule{0.05em}{0.2em}{0.2em}
    Cosine& 95.65& 22.65& 94.68& 99.50& 1.53 &99.88\\
    Cosine\textsubscript{Contrast} & 98.38 & 8.64 & 96.36 & \bf99.87 & 1.93 & \bf99.96 \\
\bf Cosine\textsubscript{VI}& \bf98.87 & \bf6.62\hspace{0.5em} & \bf98.06 & 99.57 &\bf1.43\hspace{0.5em} &99.88 \\

\specialrule{0.05em}{0.2em}{0.2em}
    Energy& 89.80& 67.00 &86.53& 93.30& 56.70&98.63 \\    
    Energy\textsubscript{Contrast}& 84.93& 63.16 &69.29& 94.44& 44.46&98.86 \\    
\bf Energy\textsubscript{VI}& \bf92.79 & \bf51.25 &\bf89.26 &\bf 96.05 & \bf27.97 &\bf99.12 \\

\specialrule{0.05em}{0.2em}{0.2em}
\specialrule{0.15em}{0.2em}{0.1em}

&   \multicolumn{3}{c}{\bf TREC-10} & \multicolumn{3}{c}{\bf 20NG}\\
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
Methods & \makecell[c]{AUROC  \uparrow}  & \makecell[c]{FAR@95  \downarrow}& \makecell[c]{AUPR \uparrow} &  \makecell[c]{AUROC  \uparrow}  & \makecell[c]{FAR@95 \downarrow} & \makecell[c]{AUPR \uparrow}\\
\specialrule{0.1em}{0.1em}{0.1em}
    MSP&  97.94 & 8.43 & 89.26 & \bf93.89 & 30.49& \bf87.39 \\
    MSP\textsubscript{Contrast}&  98.43 & 4.06 & \bf91.19 & 93.19 & 28.00& 83.17 \\
\bf MSP\textsubscript{VI}& \bf98.91 & \bf2.77 &90.39 & 93.29  & \bf25.61 & 80.09\\
\specialrule{0.05em}{0.2em}{0.2em}
    Maha& 98.99 & 4.87 & 95.11& 98.39 & 7.77&95.91 \\
    Maha\textsubscript{Contrast}& \bf99.57 & 0.97 & \bf98.59& 98.78 & 5.89 &97.29 \\
\bf Maha\textsubscript{VI}& 99.46 & \bf0.79& 97.67 & \bf99.80 & \bf0.61\hspace{0.5em} &\bf98.93 \\
\specialrule{0.05em}{0.2em}{0.2em}
     Cosine& 98.89 & 3.96 & 94.54& 97.73 & 10.84 & 88.71\\
     Cosine\textsubscript{Contrast}& 99.14 & 1.42 & 93.34& 98.03 & 8.86 & 95.27\\
\bf Cosine\textsubscript{VI}& \bf99.36 & \bf1.19 &\bf96.09 & \bf99.39 &\bf 2.92\hspace{0.5em} &\bf97.19 \\
\specialrule{0.05em}{0.2em}{0.2em}
    Energy& 97.19 & 10.07 &82.16 & 95.76& 17.93&\bf88.71 \\      
    Energy\textsubscript{Contrast}& 98.45 & 4.73 &\bf91.18 & \bf96.04& \bf15.70&88.62 \\ 
\bf Energy\textsubscript{VI}& \bf99.21& \bf2.84&90.84 & 94.34 & 17.04 &79.67\\

\specialrule{0.05em}{0.2em}{0.2em}
\specialrule{0.15em}{0.2em}{0.1em}

 \multirow{2}*{Average} &   \multicolumn{2}{c}{AUROC \uparrow}  & \multicolumn{2}{c}{FAR@95 \downarrow} & \multicolumn{2}{c}{AUPR \uparrow}\\
  \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7}   
 
\specialrule{0.05em}{0.2em}{0.2em}
avg. (MSP / Maha / Cosine / Energy) & 
\multicolumn{2}{c}{94.00 / 98.78 / 97.94 / 94.01} &
\multicolumn{2}{c}{36.76 / 6.21 / 9.75 / 37.93} & 
\multicolumn{2}{c}{\textbf{90.46} / 97.07 / 94.45 / 89.01}\\       

avg.\textsubscript{Contrast} (MSP / Maha / Cosine / Energy) & 
\multicolumn{2}{c}{92.79 / 99.17 / 98.86 / 93.47} &
\multicolumn{2}{c}{35.04 / 3.93 / 5.21 / 32.01} & 
\multicolumn{2}{c}{85.65 / 97.43 / 96.23 / 86.99}\\



\textbf{avg.\textsubscript{VI}} (MSP / Maha / Cosine / Energy)& 
\multicolumn{2}{c}{\textbf{95.25} / \textbf{99.62} / \textbf{99.30} / \textbf{95.60}} & 
\multicolumn{2}{c}{\textbf{27.00} / \textbf{1.31} / \textbf{3.04} / \textbf{24.78}} & 
\multicolumn{2}{c}{89.83 / \textbf{98.77} / \textbf{97.81} / \textbf{89.72}} \\
% \colorbox{lightgray}{

\specialrule{0.15em}{0.1em}{0.2em}
\end{tabular}
}
\caption{\label{tab:main}
    Main results of our proposed framework. MSP, Maha, Energy, and Cosine are baseline methods trained with the discriminative loss, while each corresponding method with the \emph{VI} subscript denotes the model trained with our VI framework. The \emph{Contrast} subscript denotes the method proposed by \citet{zhou2021contrastive}.
    % The gray cell color indicates our VI framework achieves better results than the baselines. 
    The best result is marked in bold. 
    % Models are fine-tuned on the training set of each ID dataset. 
    At the bottom row, averaged results across four ID datasets are included. All the reported results are presented in percentage values.
}
\end{table*}



% \begin{table*}[ht!]
% \centering
% \scalebox{0.68}{
% \begin{tabular}{cllllll}
% \specialrule{0.15em}{0.1em}{0.1em}

%  &  \multicolumn{3}{c}{\bf SST-2} & \multicolumn{3}{c}{\bf IMDB}\\
%  \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
% Methods & \makecell[c]{AUROC  \uparrow}  & \makecell[c]{FAR@95  \downarrow}& \makecell[c]{AUPR \uparrow} &  \makecell[c]{AUROC  \uparrow}  & \makecell[c]{FAR@95 \downarrow} & \makecell[c]{AUPR \uparrow}\\
% \specialrule{0.1em}{0.1em}{0.1em}
%     MSP&  89.85& 66.20 & 86.40 & 94.30& 41.90 & 98.80 \\
% \bf MSP\textsubscript{VI}& 92.85 {\color{teal}(+3.00)} & 51.58 {\color{teal}(+14.62)}&89.72 {\color{teal}(+3.32)}& 95.95 {\color{teal}(+1.65)}& 28.03 {\color{teal}(+13.87)}&99.12 {\color{teal}(+0.32)}\\
% \specialrule{0.05em}{0.2em}{0.2em}
%     Maha& 97.98& 11.50 & 97.30 & 99.67& 0.70 & 99.95 \\
% \bf Maha\textsubscript{VI}& \textbf{99.33} {\color{teal}(+1.35)}& \textbf{3.62}\hspace{0.5em}   {\color{teal}(+7.88)}&\textbf{98.52} {\color{teal}(+1.22)}& \textbf{99.90} {\color{teal}(+0.23)}& \textbf{0.21}\hspace{0.5em} {\color{teal}(+0.49)}& \textbf{99.97} {\color{teal}(+0.02)} \\
% \specialrule{0.05em}{0.2em}{0.2em}
%     Cosine& 95.65& 22.65& 94.68& 99.50& 1.53 &99.88\\
% \bf Cosine\textsubscript{VI}& 98.87 {\color{teal}(+3.22)}& 6.62\hspace{0.5em} {\color{teal}(+16.03)}& 98.06 {\color{teal}(+3.38)}& 99.57 {\color{teal}(+0.07)}&1.43\hspace{0.5em} {\color{teal}(+0.10)}&99.88 ( 0.00)\\

% \specialrule{0.05em}{0.2em}{0.2em}
%     Energy& 89.80& 67.00 &86.53& 93.30& 56.70&98.63 \\       
% \bf Energy\textsubscript{VI}& 92.79 {\color{teal}(+2.99)}& 51.25 {\color{teal}(+15.75)}&89.26 {\color{teal}(+2.73)}& 96.05 {\color{teal}(+2.75)}& 27.97 {\color{teal}(+28.73)}&99.12 {\color{teal}(+0.49)}\\

% \specialrule{0.05em}{0.2em}{0.2em}
% \specialrule{0.15em}{0.2em}{0.1em}

% &   \multicolumn{3}{c}{\bf TREC-10} & \multicolumn{3}{c}{\bf 20NG}\\
%  \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
% Methods & \makecell[c]{AUROC  \uparrow}  & \makecell[c]{FAR@95  \downarrow}& \makecell[c]{AUPR \uparrow} &  \makecell[c]{AUROC  \uparrow}  & \makecell[c]{FAR@95 \downarrow} & \makecell[c]{AUPR \uparrow}\\
% \specialrule{0.1em}{0.1em}{0.1em}
%     MSP&  97.94 & 8.43 & 89.26 & 93.89 & 30.49& 87.39 \\
% \bf MSP\textsubscript{VI}& 98.91 {\color{teal}(+0.97)}& 2.77 {\color{teal}(+5.66)}&90.39 {\color{teal}(+1.13)}& 93.29 (-0.60) & 25.61 {\color{teal}(+4.88)}& 80.09 (-7.3)\\
% \specialrule{0.05em}{0.2em}{0.2em}
%     Maha& 98.99 & 4.87 & 95.11& 98.39 & 7.77&95.91 \\
% \bf Maha\textsubscript{VI}& \textbf{99.46} {\color{teal}(+0.47)}& \textbf{0.79} {\color{teal}(+4.08)}& \textbf{97.67} {\color{teal}(+2.56)}& \textbf{99.80} {\color{teal}(+1.41)}& \textbf{0.61}\hspace{0.5em} {\color{teal}(+7.16)}&\textbf{98.93} {\color{teal}(+3.02)}\\
% \specialrule{0.05em}{0.2em}{0.2em}
%      Cosine& 98.89 & 3.96 & 94.54& 97.73 & 10.84 & 88.71\\
% \bf Cosine\textsubscript{VI}& 99.36 {\color{teal}(+0.47)}& 1.19 {\color{teal}(+2.77)}&96.09 {\color{teal}(+1.55)}& 99.39 {\color{teal}(+1.66)}& 2.92\hspace{0.5em} {\color{teal}(+7.92)}&97.19 {\color{teal}(+8.48)}\\
% \specialrule{0.05em}{0.2em}{0.2em}
%     Energy& 97.19 & 10.07 &82.16 & 95.76& 17.93&88.71 \\       
% \bf Energy\textsubscript{VI}& 99.21 {\color{teal}(+2.02)}& 2.84 {\color{teal}(+7.23)}&90.84 {\color{teal}(+8.68)}& 94.34 (-1.42)& 17.04 {\color{teal}(+0.89)}&79.67 (-9.04)\\

% \specialrule{0.05em}{0.2em}{0.2em}
% \specialrule{0.15em}{0.2em}{0.1em}

%  \multirow{2}*{Average} &   \multicolumn{2}{c}{AUROC \uparrow}  & \multicolumn{2}{c}{FAR@95 \downarrow} & \multicolumn{2}{c}{AUPR \uparrow}\\
%   \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7}   
 
% \specialrule{0.05em}{0.2em}{0.2em}
% avg. (MSP / Maha / Cosine / Energy) & 
% \multicolumn{2}{c}{94.00 / 98.78 / 97.94 / 94.01} &
% \multicolumn{2}{c}{36.76 / 6.21 / 9.75 / 37.93} & 
% \multicolumn{2}{c}{\textbf{90.46} / 97.07 / 94.45 / 89.01}\\       

% \textbf{avg.\textsubscript{VI}} (MSP / Maha / Cosine / Energy)& 
% \multicolumn{2}{c}{\textbf{95.25} / \textbf{99.62} / \textbf{99.30} / \textbf{95.60}} & 
% \multicolumn{2}{c}{\textbf{27.00} / \textbf{1.31} / \textbf{3.04} / \textbf{24.78}} & 
% \multicolumn{2}{c}{89.83 / \textbf{98.77} / \textbf{97.81} / \textbf{89.72}} \\
% % \colorbox{lightgray}{

% \specialrule{0.15em}{0.1em}{0.2em}
% \end{tabular}
% }
% \caption{\label{tab:main}
%     Main results of our proposed variational inference (VI) framework. MSP, Maha, Energy, and Cosine are baseline methods trained with the discriminative loss while each corresponding method with the \emph{VI} subscript denotes the model trained with our VI framework.
%     % The gray cell color indicates our VI framework achieves better results than the baselines. 
%     The best result is marked in bold. Models are fine-tuned on the training set of each in-distribution (ID) dataset, i.e., SST-2, IMDB, TREC-10, and 20NG. At the bottom row, averaged results across four ID datasets are included. Results for each metric are averaged across $8$ OOD test datasets. All results are in $100\%$.
% }
% \end{table*}

\subsection{Main Results}
% We conduct extensive experiments on the four in-distribution tasks described in Subsection~(\ref{sec:dataset}) and compare our proposed variational framework against baselines trained with $p(y|x)$.
% Results are summarized in Table~\ref{tab:main}. 
% We demonstrate the versatility of our proposed VI-OOD detection framework by considering four in-distribution (ID) datasets in addition to the other four out-distribution datasets, i.e., the model trained on each ID dataset will be evaluated on seven OOD test sets (except SST-2 and IMDB). Averaged Results are summarized in Table~\ref{tab:main} and detailed results are presented in the appendix~\ref{sec:all_results}.
To showcase the adaptability of our VI-OOD detection framework, we evaluate it on comprehensive datasets and compare it with competitive baselines. 
% Each model trained on an ID dataset is tested on seven OOD test sets. 
% The summarized averaged results can be found in Table~\ref{tab:main}, while comprehensive results are provided in Appendix~\ref{sec:all_results}.
The summarized averaged results can be found in Table~\ref{tab:main}.

% , while comprehensive results are provided in Appendix~\ref{sec:all_results}.

\paragraph{VI-OOD benefits a diverse collection of tasks and OOD score functions.}
% According to Table~\ref{tab:main}, 
% A salient observation is that for all the compared OOD score functions, our proposed approach can consistently achieve better performance. For example, for the best-performing baseline -- the Maha method, our method reduces the average FAR@95 from $6.21\%$ to $1.31\%$, which leads to a $78.9\%$ relative increase. 
% For the second best baseline--Cosine score function, the improvement of our method is also significant, i.e., reducing average FAR@95 from $9.75\%$ to $3.04\%$. 
% Besides the improvements on FAR@95, performance gains on AUROC are also significant. For example, the average AUROC sore of the Cosine method increases from $97.94\%$ to $99.3\%$.
% Considering that our method requires no real OOD examples involved, these results are very encouraging.

According to Table~\ref{tab:main}, one notable observation is that our proposed approach consistently outperforms all compared baselines in terms of the overall average performance. This can be observed across various metrics. For instance, when comparing our method to the best-performing baseline, the Maha method, we achieve a significant reduction in the average FAR@95 from $6.21\%$ to $1.31\%$, resulting in a relative increase of $78.9\%$. Similarly, for the second best baseline, the Cosine score function, our method demonstrates substantial improvement by reducing the average FAR@95 from $9.75\%$ to $3.04\%$. Moreover, there are significant performance gains in terms of AUROC as well. For example, the average AUROC score for the Cosine method increases from $97.94\%$ to $99.3\%$ with the use of our method. It is worth noting that our method achieves these improvements without the need for real OOD examples, which makes these results even more encouraging.
% Looking into each of the four ID datasets, it can be seen that detecting OOD test examples on the model trained on TREC-10 is much easier than other datasets, i.e., all OOD score functions achieve the AUROC score above $97\%$. Improvements upon these competitive results can be challenging. Nevertheless, our method also achieves better performance for all four score functions. In particular, The AUROC score of Energy is improved from $97.19\%$ to $99.21\%$ and the corresponding FAR@95 score is reduced from $10.07\%$ to $2.84\%$. For the Maha method on TREC-10, our method reduces the FAR@95 score to $0.79\%$ which is near perfect.
Upon closer examination of each of the four in-distribution (ID) datasets, it becomes apparent that detecting out-of-distribution (OOD) test examples using the model trained on TREC-10 is comparatively easier than with the other datasets. In fact, all OOD score functions achieve AUROC scores above $97\%$. Improving upon these already competitive results poses a significant challenge. However, our method still manages to outperform all four score functions on TREC-10. Notably, for the Energy score function, our method enhances the AUROC score from $97.19\%$ to $99.21\%$, while simultaneously reducing the FAR@95 score from $10.07\%$ to $2.84\%$. Furthermore, for the Maha method on TREC-10, our method achieves a near-perfect FAR@95 score of $0.79\%$.

\begin{table*}[ht!]
\centering
\scalebox{0.9}{
\begin{tabular}{ccccccc}
\specialrule{0.15em}{0.1em}{0.1em}

 &  \multicolumn{3}{c}{\bf SST-2} & \multicolumn{3}{c}{\bf TREC-10}\\
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
Methods & \makecell[c]{AUROC  \uparrow}  & \makecell[c]{FAR@95  \downarrow}& \makecell[c]{AUPR \uparrow} &  \makecell[c]{AUROC  \uparrow}  & \makecell[c]{FAR@95 \downarrow} & \makecell[c]{AUPR \uparrow}\\
\specialrule{0.1em}{0.1em}{0.1em}

    MSP&  78.22 & 70.40 & 74.34 & \bf99.29& \bf0.64 & \bf98.79 \\
\bf MSP\textsubscript{VI}& \bf 83.05 & \bf65.32 &\bf 69.54 &  98.69 & 5.69 &94.48 \\
\specialrule{0.05em}{0.2em}{0.2em}
    Maha& 46.08& 84.41 & 47.34 & 84.41& 71.94 & 64.13 \\
\bf Maha\textsubscript{VI}& \bf95.41 & \bf12.47\hspace{0.5em} &\bf85.38 & \bf99.96 & \bf0.12\hspace{0.5em} & \bf99.39  \\
\specialrule{0.05em}{0.2em}{0.2em}
    Cosine& 89.24& 26.52& 79.47& 98.24& 11.06 &93.05\\
\bf Cosine\textsubscript{VI}& \bf95.95 & \bf7.21\hspace{0.5em} & \bf85.70 & \bf100 &\bf0\hspace{0.5em} &\bf99.92 \\

\specialrule{0.05em}{0.2em}{0.2em}
    Energy& 70.13& 67.78 &64.87& \bf99.86& \bf0.14&\bf99.27 \\        
\bf Energy\textsubscript{VI}& \bf80.16 & \bf66.90 &\bf65.76 &98.64 & 7.40 &92.44 \\

\specialrule{0.05em}{0.2em}{0.2em}
\end{tabular}
}
\caption{\label{tab:llama}
    Results of our proposed framework on LLaMA-2-7B, fine-tuned with a classification head.  
    % The gray cell color indicates our VI framework achieves better results than the baselines. 
    The best result is marked in bold. 
    % Models are fine-tuned on the training set of each ID dataset. 
    All the reported results are presented in percentage values.
}
\end{table*}
% \paragraph{Our method outperforms baselines on larger decoder-only models.} To further verify the effectiveness of our method, we conduct experiments on SST-2 and TREC-10 with LLaMA-2-7B. We use \emph{LlamaForSequenceClassification} provided by Hugginface's transformers package~\cite{wolf-etal-2020-transformers} to train the in-distribution classifier.

\paragraph{Superior Performance of Our Method with Large Decoder-Only Models.} To further validate our method's efficacy, we conduct experiments on SST-2 and TREC-10 using LLaMA-2-7B. For training the in-distribution classifier, we utilize \emph{LlamaForSequenceClassification} from the Hugging Face transformers package~\cite{wolf-etal-2020-transformers}.

% Results are present in Table~\ref{tab:llama}. It can be seen that when SST-2 as the ID dataset, our method outperforms baselines by a large margin on all three metrics. For TREC-10, our method boosts Maha and Cosine OOD scores to near-perfect performance. However, for the logit-based OOD scores, i.e., MSP and Energy, our method achieves slightly poorer performance compared to the corresponding baselines. It may be because Maha and Consine can benefit more from richer information in the sentence representation, but richer information leads to more ambiguity in the logits.
Results are presented in Table~\ref{tab:llama}. As shown, when using SST-2 as the in-distribution (ID) dataset, our method significantly outperforms the baselines across all three metrics. In the case of TREC-10, our method elevates the Mahalanobis (Maha) and Cosine OOD scores to nearly perfect levels. However, for logit-based OOD scores, specifically MSP and Energy, our method demonstrates slightly inferior performance relative to the respective baselines. This discrepancy may stem from the fact that Maha and Cosine benefit more from the enriched information in sentence representations, whereas this richer information introduces more ambiguity in the logits.




% \paragraph{VI-OOD narrows the gap between different OOD score functions.}

\begin{figure}
    \centering
    \scalebox{1.}{
    \includegraphics[width=8cm,height=6cm]{figures/heatmap.png}
    % \includegraphics[width=1\linewidth]{./f}
    }
    \caption{Heatmap of the hidden state combination factor $s$. The horizontal axis stands for four ID tasks and the vertical axis represents the layer number.}
    \label{fig:factor}
\end{figure}
\subsection{ID Classification Performance}
In this subsection, we investigate the ID classification performance. Besides the binary ID \emph{vs.} OOD task, OOD detection also concerns the ID classification task. We summarize the test accuracy of the corresponding ID test sets for the four ID datasets in Table~\ref{tab:test_acc}. It can be seen that for 20NG, SST-2, TREC-10, and IMDB, ID test performances are very similar and all the gaps are lower than $1\%$.
Therefore, models trained with our proposed $p(x, y)$ target do not bring significant detrimental impacts to ID classification. However, although we consider these gaps can be ignored in practical applications, it also indicates that our method can be further improved in further works.


\begin{table}
\centering
% \large
% \small
\scalebox{.8}{
\begin{tabular}{c|cccc}
\specialrule{0.08em}{0.1em}{0.1em}
Test Accuracy &SST-2&IMDB&TREC-10&20NG\\
% &Methods 
\specialrule{0.05em}{0.1em}{0.05em}
$p(y|x)$&96.21&95.33&97.8&93.99 \\
                    
\specialrule{0.05em}{0.1em}{0.05em}

$p(x, y)$&96.38&94.54&97.0&93.35 \\
\specialrule{0.1em}{0.1em}{0.1em}
\end{tabular}
}
\caption{\label{tab:test_acc}
% A pilot study of two state-of-the-art OOD intent detection approaches on few-shot OOD detection. 
Performance comparison of the ID K-class classifier for different training objectives. $p(y|x)$ is the commonly used discriminative objective and $p(x, y)$ is our proposed objective.
% For the 75\% setting, the top 2 results for each metric are marked in bold.
}
\end{table}
\subsection{The Combination Factor $s$}
% At last, we analyze the proposed combination vector $\mathbf{s}$. We plot the heatmap of the learned $\mathbf{s}$ for in-distribution (ID) tasks in Figure~\ref{fig:factor}. It can be seen that for different ID tasks, the hidden state combination patterns are very different, indicating that our proposed combination vector could automatically learn suitable combination policies for different ID tasks. It verifies the flexibility of our proposed framework in utilizing the powerful hidden states of pre-trained models.
Finally, we analyze the learned combination vector $\mathbf{s}$ in our framework. We visualize the heatmap of the learned $\mathbf{s}$ for the in-distribution (ID) tasks in Figure~\ref{fig:factor}. It is evident that the hidden state combination patterns vary significantly across different ID tasks. This observation confirms that our proposed combination vector can automatically adapt and learn appropriate combination policies for distinct ID tasks. This analysis provides further evidence of the flexibility of our framework in effectively leveraging the potent hidden states of pre-trained models.
